Generating Adversarial Computer Programs using Optimized Obfuscations

Machine learning (ML) models that learn and predict properties of computer programs are increasingly being adopted and deployed. These models have demonstrated success in applications such as auto-completing code, summarizing large programs, and detecting bugs and malware in programs. In this work, we investigate principled ways to adversarially perturb a computer program to fool such learned models, and thus determine their adversarial robustness. We use program obfuscations, which have conventionally been used to avoid attempts at reverse engineering programs, as adversarial perturbations. These perturbations modify programs in ways that do not alter their functionality but can be crafted to deceive an ML model when making a decision. We provide a general formulation for an adversarial program that allows applying multiple obfuscation transformations to a program in any language. We develop first-order optimization algorithms to efficiently determine two key aspects -- which parts of the program to transform, and what transformations to use. We show that it is important to optimize both these aspects to generate the best adversarially perturbed program. Due to the discrete nature of this problem, we also propose using randomized smoothing to improve the attack loss landscape to ease optimization. We evaluate our work on Python and Java programs on the problem of program summarization. We show that our best attack proposal achieves a $52\%$ improvement over a state-of-the-art attack generation approach for programs trained on a seq2seq model. We further show that our formulation is better at training models that are robust to adversarial attacks.

==> figures.tex <==
%<*mainfig>
\begin{figure}[tb]
        \centering
        \resizebox{0.85\textwidth}{!}{
            \includegraphics[width=0.9\textwidth ]{img/transforms.png}
        }
            \caption{\small{ (a) A sample program $\prog$ containing a function {\small \texttt{foo}} (b) $\prog$ contains five \textit{sites} which can be transformed - two \replace sites corresponding to local variables \fcolorbox{black}{bisque}{b} and \fcolorbox{black}{lime}{r}, and three \insertt sites at locations {\small \texttt{I1}, \texttt{I2}, \texttt{I3}}. $\Omega$ is a vocabulary of tokens which can be used for the transformations. (c) This is a \textit{perturbed program} with the tokens {\small \texttt{world}} and {\small \texttt{set}} from $\Omega$ used to replace tokens \texttt{b} and at location {\small \texttt{I3}}. These transformations do not change the original functionality of $\prog$, but cause an incorrect prediction {\small {\small \texttt{delete}}} (d) Examples of two site selection vectors $\mathbf z^\mathrm{i}$, $\mathbf z^\mathrm{ii}$ selecting different components. $\mathbf z_i = 1$ for a location $i$ signifies that the $i$th token in $\prog$ is selected to be optimally transformed. $\mathbf z^\mathrm{i}$ corresponds to the perturbed program in (c).}}
        \label{transforms}
\end{figure}
%</mainfig>

%<*resultstable>
    \input{table.tex}
%</resultstable>

%<*resultsplots>
    \begin{figure}[htb]
    \hspace*{-0.7in}
    \centering % <-- added
    {
    % \begin{subfigure}{\wdd\textwidth}
    %     \includegraphics[width=\linewidth]{img/py150-z_o_1.png}
    %     \label{fig:1}
    % \end{subfigure}
    % \begin{subfigure}{\wdd\textwidth}
    %   \includegraphics[width=\linewidth]{img/py150-z_o_5.png}
    %   \label{fig:2}
    % \end{subfigure}
    % \begin{subfigure}{0.4\textwidth}
    %   \includegraphics[width=\linewidth]{img/py150-asr_vs_sites.png}
    % \end{subfigure}
    % \begin{subfigure}{\wdd\textwidth}
    %   \includegraphics[width=\linewidth]{img/javasmall-z_o_1.png}
    %   \label{fig:4}
    % \end{subfigure}
    % \begin{subfigure}{\wdd\textwidth}
    %   \includegraphics[width=\linewidth]{img/javasmall-z_o_5.png}
    %   \label{fig:5}
    % \end{subfigure}
    % %\begin{subfigure}{0.4\textwidth}
    %  \includegraphics[width=\linewidth]{img/javasmall-asr_vs_sites.png}
    %  \label{fig:6}
    %\end{subfigure}
}
\caption{Dependence of Attack Success Rate (ASR) on two parameters -- number of iterations the optimization process is run for, and the perturbation strength ($k$). The first two plots in each row show the dependence as the number of iterations increase. The third plot in each row shows how the ASR varies with an increase in the \# of sites allowed to be perturbed.}
\label{fig:images}
\end{figure}

%</resultsplots>


%<*example1>
    \begin{figure}[tb]
    \hspace*{-0.5in}
    {
        \begin{subfigure}{0.6\textwidth}
            \includegraphics[width=\linewidth]{img/example1.png}
            \caption{Effect of optimizing $z$}
            \label{fig:ex1}
        \end{subfigure}
        \begin{subfigure}{0.6\textwidth}
          \includegraphics[width=\linewidth]{img/example2.png}
          \caption{Effect of optimizing $z$ and smoothing the loss function}
          \label{fig:ex2}
        \end{subfigure}
    }
\caption{\small{Example adversarial attacks on two programs from the dataset evaluated in this work. The goal is for the transformations to change the prediction seen in the unperturbed setting. In \ref{fig:ex1}, the best token replacement at a randomly selected site (\texttt{virtualname}) is incapable of changing the classifier's decision. In \ref{fig:ex2}, the prediction does not change despite optimizing $z$. Smoothing then enables searching for a better replacement token (\texttt{datetime}).}}
\end{figure}
%</example1>

%<*example2>
    \begin{wrapfigure}{r}{0.45\textwidth}
        \resizebox{0.45\textwidth}{!}{
        \includegraphics[width=\linewidth]{img/example1.png}
        }
        \caption{\small{The advantage of our formulation when compared to the state-of-the-art.}}
        \label{fig:ex1solo}
        
    \end{wrapfigure}
%</example2>


%<*loss>
    \begin{wrapfigure}[19]{r}{0.6\textwidth}
      \hspace*{-8mm}   \begin{minipage}[t]{0.38\textwidth}
    \includegraphics[width=\textwidth]{img/loss_plot_sign_lossvals_nosmooth.json.png}
    \vspace*{-3mm}
            \subcaption{~}
            \label{fig:loss_nonsmooth}
        \end{minipage}
         \hspace*{-8mm}
        \begin{minipage}[t]{0.38\textwidth}
         \includegraphics[width=\textwidth]{img/loss_plot_sign_lossvals_0.01.json.png}
          \vspace*{-3mm}
            \subcaption{~}
            \label{fig:loss_smooth}
        \end{minipage}
        \caption{\small{The original loss landscape for a sample program \eqref{fig:loss_nonsmooth}. Randomized smoothing produces a flatter and smoother loss landscape \eqref{fig:loss_smooth}. We plot the loss along the space determined by the vector {\small$(\alpha.\mathrm{sgn}(\nabla_xf(x))+\beta.\mathrm{Rademacher}(0.5))$} for $\alpha$, $\beta$ $\in$ $[-0.05, 0.05]$}~\citep{engstrom2018evaluating}}
        \label{fig:loss}
    \end{wrapfigure}
%</loss>

%<*iters-sites>
    \begin{wrapfigure}[15]{r}{0.65\textwidth}
    \vspace*{-5mm}
        \begin{minipage}[t]{0.33\textwidth}
     \hspace*{-2mm}       \includegraphics[width=\textwidth]{img/py150-z_o_5.png}
     \vspace*{-1mm}
            \subcaption{~}
            \label{fig:iters}
        
        \end{minipage}
        \begin{minipage}[t]{0.33\textwidth}
             \hspace*{-1mm}   \includegraphics[width=\textwidth]{img/py150-asr_vs_sites.png}
                  \vspace*{-1mm}
            \subcaption{~}
            \label{fig:sites}
        
        \end{minipage}
        \captionsetup{skip=\dimexpr\abovecaptionskip-10pt}
        \caption{\small{ASRs of our approaches and {\baseline} against  the number of optimization iterations \eqref{fig:iters} and  \textnormal{\ptst} of an attacker \eqref{fig:sites}.}}
    \end{wrapfigure}
%</iters-sites>

%<*robustresults>
\begin{wraptable}[12]{r}{0.45\textwidth}
    \renewcommand{\arraystretch}{1.2}
	\centering
	\resizebox{0.35\textwidth}{!}{
	\begin{tabular}{l| l l l l}
	\multirow{2}{*}{\textbf{Train}} & \multicolumn{3}{c}{\textbf{Attack} (ASR)}\\
	& \baselinesmall & \ao & \aors \\\hline
	{\small{No AT}} &19.87 &23.16 & 30.25\\
	\baselinesmall &17.99 &18.87 & 19.11\\
	%\ao &x &x & x\\
	\textbf{\aors} &\textbf{12.73} &\textbf{13.01} & \textbf{13.75}\\
	\end{tabular}
	}
	\caption{\small{We employ an AT setup to train \textsc{seq2seq} with the attack formulation we propose. Lower the ASR, higher the robustness to adversarial attacks. Training under \aors attacks provides best robustness results.}
	%	\vspace*{-10mm}
	}
	\label{tbl:robustness}
		%\vspace*{-50mm}
\end{wraptable}
%</robustresults>



==> full_table.tex <==
 \renewcommand{\arraystretch}{1.25}
	\begin{table}[]
	\hspace*{-0.6in}
	\centering
	\resizebox{1.25\textwidth}{!}{
	\begin{tabular}{l  c r c r | c r c r | c r c r | c r c r}
	\toprule
	\multirow{3}{*}{\textbf{Method}} & \multicolumn{8}{c|}{\textbf{Python}} & \multicolumn{8}{c}{\textbf{Java}} \\ 
 		& \multicolumn{4}{c}{\textbf{$\boldsymbol{k=1}$ site}} &  \multicolumn{4}{c|}{\textbf{$\boldsymbol{k=5}$  sites}} &  \multicolumn{4}{c}{\textbf{$\boldsymbol{k=1}$ site}} &  \multicolumn{4}{c}{\textbf{$\boldsymbol{k=5}$ sites}}\\ \cline{2-17}
 		& \multicolumn{2}{c}{\textbf{ASR}} & \multicolumn{2}{c|}{\textbf{F1}} & 		\multicolumn{2}{c}{\textbf{ASR}} & \multicolumn{2}{c|}{\textbf{F1}} & 		\multicolumn{2}{c}{\textbf{ASR}} & \multicolumn{2}{c|}{\textbf{F1}} & 		\multicolumn{2}{c}{\textbf{ASR}} & \multicolumn{2}{c}{\textbf{F1}} \\ \hline
 	No attack & 0.03 &   & 99.82 &   & 0.03 &   & 99.82 &   & 0.00 &   & 99.90 &   & 0.00 &   & 99.90 &  \\ 

Random replace & 0.03 &   & 99.82 &   & 0.03 &   & 99.82 &   & 0.00 &   & 99.90 &   & 0.00 &   & 99.90 &  \\ \hline 

\textsc{Baseline*} & 19.87 &   & 78.18 &   & 37.50 &   & 59.54 &   & 21.41 &   & 72.39 &   & 28.43 &   & 56.90 &  \\ \hline 

\ao & 23.16 & \textcolor{blue}{+3.29}~$\begingroup\color{green}\blacktriangle\endgroup$ & 74.78 & \textcolor{blue}{-3.40}~$\begingroup\color{green}\blacktriangle\endgroup$ & 43.53 & \textcolor{blue}{+6.03}~$\begingroup\color{green}\blacktriangle\endgroup$ & 53.75 & \textcolor{blue}{-5.79}~$\begingroup\color{green}\blacktriangle\endgroup$ & 22.60 & \textcolor{blue}{+1.19}~$\begingroup\color{green}\blacktriangle\endgroup$ & 70.39 & \textcolor{blue}{-2.00}~$\begingroup\color{green}\blacktriangle\endgroup$ & 29.06 & \textcolor{blue}{+0.63}~$\begingroup\color{green}\blacktriangle\endgroup$ & 56.05 & \textcolor{blue}{-0.85}~$\begingroup\color{green}\blacktriangle\endgroup$\\ 

\jo & 23.32 & \textcolor{blue}{+3.45}~$\begingroup\color{green}\blacktriangle\endgroup$ & 74.56 & \textcolor{blue}{-3.62}~$\begingroup\color{green}\blacktriangle\endgroup$ & 41.95 & \textcolor{blue}{+4.45}~$\begingroup\color{green}\blacktriangle\endgroup$ & 56.06 & \textcolor{blue}{-3.48}~$\begingroup\color{green}\blacktriangle\endgroup$ & 20.55 & \textcolor{red}{-0.86}~$\begingroup\color{red}\blacktriangledown\endgroup$ & 71.89 & \textcolor{blue}{-0.50}~$\begingroup\color{green}\blacktriangle\endgroup$ & 27.17 & \textcolor{red}{-1.26}~$\begingroup\color{red}\blacktriangledown\endgroup$ & 58.15 & \textcolor{red}{+1.25}~$\begingroup\color{red}\blacktriangledown\endgroup$\\ 

\begin{tabular}[l]{@{}l@{}}\ao + RS\end{tabular} & 30.25 & \textcolor{blue}{+10.38}~$\begingroup\color{green}\blacktriangle\endgroup$ & 69.52 & \textcolor{blue}{-8.66}~$\begingroup\color{green}\blacktriangle\endgroup$ & 51.68 & \textcolor{blue}{+14.18}~$\begingroup\color{green}\blacktriangle\endgroup$ & 47.92 & \textcolor{blue}{-11.62}~$\begingroup\color{green}\blacktriangle\endgroup$ & 23.91 & \textcolor{blue}{+2.50}~$\begingroup\color{green}\blacktriangle\endgroup$ & 69.51 & \textcolor{blue}{-2.88}~$\begingroup\color{green}\blacktriangle\endgroup$ & 32.78 & \textcolor{blue}{+4.35}~$\begingroup\color{green}\blacktriangle\endgroup$ & 53.18 & \textcolor{blue}{-3.72}~$\begingroup\color{green}\blacktriangle\endgroup$\\ 

\begin{tabular}[l]{@{}l@{}}\jo + RS\end{tabular} & 23.95 & \textcolor{blue}{+4.08}~$\begingroup\color{green}\blacktriangle\endgroup$ & 74.24 & \textcolor{blue}{-3.94}~$\begingroup\color{green}\blacktriangle\endgroup$ & 48.70 & \textcolor{blue}{+11.20}~$\begingroup\color{green}\blacktriangle\endgroup$ & 51.55 & \textcolor{blue}{-7.99}~$\begingroup\color{green}\blacktriangle\endgroup$ & 23.03 & \textcolor{blue}{+1.62}~$\begingroup\color{green}\blacktriangle\endgroup$ & 70.63 & \textcolor{blue}{-1.76}~$\begingroup\color{green}\blacktriangle\endgroup$ & 27.44 & \textcolor{red}{-0.99}~$\begingroup\color{red}\blacktriangledown\endgroup$ & 64.33 & \textcolor{red}{+7.43}~$\begingroup\color{red}\blacktriangledown\endgroup$\\ 


\hline
\end{tabular}
\label{tbl:results}
} 
\caption{\protect\input{tablecaption.tex}}
\end{table}

==> table.tex <==
\renewcommand{\arraystretch}{1.2}
	\begin{table}[]
	\hspace*{-0in}
	\centering
	\resizebox{0.8\textwidth}{!}{
	\begin{tabular}{l  c r c r | c r c r}
	\toprule
	\multirow{2}{*}{\textbf{Method}} 		& \multicolumn{4}{c}{\textbf{$\boldsymbol{k=1}$ site}} &  \multicolumn{4}{c}{\textbf{$\boldsymbol{k=5}$  sites}}\\ 
 		& \multicolumn{2}{c}{\textbf{ASR}} & \multicolumn{2}{c|}{\textbf{F1}} & \multicolumn{2}{c}{\textbf{ASR}} & \multicolumn{2}{c}{\textbf{F1}}	\\ \hline
 	No attack & 0.00 &   & 100.00 &   & 0.00 &   & 100.00 &  \\ 

Random replace & 0.00 &   & 100.00 &   & 0.00 &   & 100.00 &  \\ \hline 

\textsc{Baseline*} & 19.87 &   & 78.18 &   & 37.50 &   & 59.54 &  \\ \hline 

\ao & 23.16 & \textcolor{blue}{+3.29}~$\begingroup\color{green}\blacktriangle\endgroup$ & 74.78 & \textcolor{blue}{-3.40}~$\begingroup\color{green}\blacktriangle\endgroup$ & 43.53 & \textcolor{blue}{+6.03}~$\begingroup\color{green}\blacktriangle\endgroup$ & 53.75 & \textcolor{blue}{-5.79}~$\begingroup\color{green}\blacktriangle\endgroup$\\ 

\jo & 23.32 & \textcolor{blue}{+3.45}~$\begingroup\color{green}\blacktriangle\endgroup$ & 74.56 & \textcolor{blue}{-3.62}~$\begingroup\color{green}\blacktriangle\endgroup$ & 41.95 & \textcolor{blue}{+4.45}~$\begingroup\color{green}\blacktriangle\endgroup$ & 56.06 & \textcolor{blue}{-3.48}~$\begingroup\color{green}\blacktriangle\endgroup$\\ 

\begin{tabular}[l]{@{}l@{}}\ao + \rsmo\end{tabular} & 30.25 & \textcolor{blue}{+10.38}~$\begingroup\color{green}\blacktriangle\endgroup$ & 69.52 & \textcolor{blue}{-8.66}~$\begingroup\color{green}\blacktriangle\endgroup$ & 51.68 & \textcolor{blue}{+14.18}~$\begingroup\color{green}\blacktriangle\endgroup$ & 47.92 & \textcolor{blue}{-11.62}~$\begingroup\color{green}\blacktriangle\endgroup$\\ 

\begin{tabular}[l]{@{}l@{}}\jo + \rsmo\end{tabular} & 23.95 & \textcolor{blue}{+4.08}~$\begingroup\color{green}\blacktriangle\endgroup$ & 74.24 & \textcolor{blue}{-3.94}~$\begingroup\color{green}\blacktriangle\endgroup$ & 48.70 & \textcolor{blue}{+11.20}~$\begingroup\color{green}\blacktriangle\endgroup$ & 51.55 & \textcolor{blue}{-7.99}~$\begingroup\color{green}\blacktriangle\endgroup$\\ 


\hline
\end{tabular}
} 
\caption{\protect\input{tablecaption.tex}}
\label{tbl:results}
\end{table}
% \renewcommand{\arraystretch}{1.25}
% 	\begin{table}[]
% 	\hspace*{-0.6in}
% 	\centering
% 	\resizebox{1.25\textwidth}{!}{
% 	\begin{tabular}{l  c r c r | c r c r | c r c r | c r c r}
% 	\toprule
% 	\multirow{3}{*}{\textbf{Method}} & \multicolumn{8}{c|}{\textbf{Python}} & \multicolumn{8}{c}{\textbf{Java}} \\ 
%  		& \multicolumn{4}{c}{\textbf{$\boldsymbol{k=1}$ site}} &  \multicolumn{4}{c|}{\textbf{$\boldsymbol{k=5}$  sites}} &  \multicolumn{4}{c}{\textbf{$\boldsymbol{k=1}$ site}} &  \multicolumn{4}{c}{\textbf{$\boldsymbol{k=5}$ sites}}\\ \cline{2-17}
%  		& \multicolumn{2}{c}{\textbf{ASR}} & \multicolumn{2}{c|}{\textbf{F1}} & 		\multicolumn{2}{c}{\textbf{ASR}} & \multicolumn{2}{c|}{\textbf{F1}} & 		\multicolumn{2}{c}{\textbf{ASR}} & \multicolumn{2}{c|}{\textbf{F1}} & 		\multicolumn{2}{c}{\textbf{ASR}} & \multicolumn{2}{c}{\textbf{F1}} \\ \hline
%  	No attack & 0.03 &   & 99.82 &   & 0.03 &   & 99.82 &   & 0.00 &   & 99.90 &   & 0.00 &   & 99.90 &  \\ 

% Random replace & 0.03 &   & 99.82 &   & 0.03 &   & 99.82 &   & 0.00 &   & 99.90 &   & 0.00 &   & 99.90 &  \\ \hline 

% \textsc{Baseline*} & 19.87 &   & 78.18 &   & 37.50 &   & 59.54 &   & 21.41 &   & 72.39 &   & 28.43 &   & 56.90 &  \\ \hline 

% \ao & 23.16 & \textcolor{blue}{+3.29}~$\begingroup\color{green}\blacktriangle\endgroup$ & 74.78 & \textcolor{blue}{-3.40}~$\begingroup\color{green}\blacktriangle\endgroup$ & 43.53 & \textcolor{blue}{+6.03}~$\begingroup\color{green}\blacktriangle\endgroup$ & 53.75 & \textcolor{blue}{-5.79}~$\begingroup\color{green}\blacktriangle\endgroup$ & 22.60 & \textcolor{blue}{+1.19}~$\begingroup\color{green}\blacktriangle\endgroup$ & 70.39 & \textcolor{blue}{-2.00}~$\begingroup\color{green}\blacktriangle\endgroup$ & 29.06 & \textcolor{blue}{+0.63}~$\begingroup\color{green}\blacktriangle\endgroup$ & 56.05 & \textcolor{blue}{-0.85}~$\begingroup\color{green}\blacktriangle\endgroup$\\ 

% \jo & 23.32 & \textcolor{blue}{+3.45}~$\begingroup\color{green}\blacktriangle\endgroup$ & 74.56 & \textcolor{blue}{-3.62}~$\begingroup\color{green}\blacktriangle\endgroup$ & 41.95 & \textcolor{blue}{+4.45}~$\begingroup\color{green}\blacktriangle\endgroup$ & 56.06 & \textcolor{blue}{-3.48}~$\begingroup\color{green}\blacktriangle\endgroup$ & 20.55 & \textcolor{red}{-0.86}~$\begingroup\color{red}\blacktriangledown\endgroup$ & 71.89 & \textcolor{blue}{-0.50}~$\begingroup\color{green}\blacktriangle\endgroup$ & 27.17 & \textcolor{red}{-1.26}~$\begingroup\color{red}\blacktriangledown\endgroup$ & 58.15 & \textcolor{red}{+1.25}~$\begingroup\color{red}\blacktriangledown\endgroup$\\ 

% \begin{tabular}[l]{@{}l@{}}\ao + \rsmo\end{tabular} & 30.25 & \textcolor{blue}{+10.38}~$\begingroup\color{green}\blacktriangle\endgroup$ & 69.52 & \textcolor{blue}{-8.66}~$\begingroup\color{green}\blacktriangle\endgroup$ & 51.68 & \textcolor{blue}{+14.18}~$\begingroup\color{green}\blacktriangle\endgroup$ & 47.92 & \textcolor{blue}{-11.62}~$\begingroup\color{green}\blacktriangle\endgroup$ & 23.91 & \textcolor{blue}{+2.50}~$\begingroup\color{green}\blacktriangle\endgroup$ & 69.51 & \textcolor{blue}{-2.88}~$\begingroup\color{green}\blacktriangle\endgroup$ & 32.78 & \textcolor{blue}{+4.35}~$\begingroup\color{green}\blacktriangle\endgroup$ & 53.18 & \textcolor{blue}{-3.72}~$\begingroup\color{green}\blacktriangle\endgroup$\\ 

% \begin{tabular}[l]{@{}l@{}}\jo + \rsmo\end{tabular} & 23.95 & \textcolor{blue}{+4.08}~$\begingroup\color{green}\blacktriangle\endgroup$ & 74.24 & \textcolor{blue}{-3.94}~$\begingroup\color{green}\blacktriangle\endgroup$ & 48.70 & \textcolor{blue}{+11.20}~$\begingroup\color{green}\blacktriangle\endgroup$ & 51.55 & \textcolor{blue}{-7.99}~$\begingroup\color{green}\blacktriangle\endgroup$ & 23.03 & \textcolor{blue}{+1.62}~$\begingroup\color{green}\blacktriangle\endgroup$ & 70.63 & \textcolor{blue}{-1.76}~$\begingroup\color{green}\blacktriangle\endgroup$ & 27.44 & \textcolor{red}{-0.99}~$\begingroup\color{red}\blacktriangledown\endgroup$ & 64.33 & \textcolor{red}{+7.43}~$\begingroup\color{red}\blacktriangledown\endgroup$\\ 


% \hline
% \end{tabular}
% \label{tbl:results}
% } 
% \caption{\protect\input{tablecaption.tex}}
% \end{table}

==> tablecaption.tex <==
{\small Our work solves two key problems to find optimal adversarial perturbations -- \stse and \stpe. The \baseline method refers to \citep{ramakrishnan2020semantic}. 
The \ptst $k$ is the maximum number of sites which an attacker can perturb. 
%We evaluate our work in two settings -- $k=1$ and $k=5$, on 
Higher the the Attack Success Rate (ASR), better the attack; the converse holds for F1 score. 
Our formulation (Eq. \ref{eq: adv_code_obfuscation}), solved using two methods -- alternate optimization (\ao) and joint optimization (\jo), along with randomized smoothing (\rsmo), shows a consistent improvement in generating adversarial programs. Differences in ASR, marked in \textcolor{blue}{blue}, are relative to \baseline. The results on a Java dataset are tabulated in Table \ref{tbl:results-java}, Appendix.}
%and \textcolor{red}{red}
